FLINT: Efficiently Leveraging High Bandwidth Flash for Capacity-Scalable LLM Inference Acceleration

LLM inference is increasingly constrained by accelerator memory capacity rather than compute throughput. This constraint is especially acute in single-accelerator and small-node inference systems, where limited on-package memory capacity restricts the size of deployable models. HBF is an emerging 3D-stacked NAND flash technology that provides multi-terabyte near-accelerator capacity, making it a promising capacity tier for storing LLM weights. However, existing HBF-based proposals face three adoption challenges: they (1) rely on coarse-grained static prefetching for LLM weights aiming to hide the microsecond-level read latency of the NAND flash device while maximizing HBF's read throughput, (2) expose NAND flash management tasks (e.g., refresh operations) to the accelerator-visible critical inference path, and (3) miss optimization opportunities to specialize and optimize the flash-management mechanisms to the workload behavior. Our goal is to design an efficient HBF substrate that integrates HBF as a memory-capacity tier alongside HBM while addressing these three challenges. To this end, we propose FLINT, a workload-driven HBF substrate for capacity-scalable LLM inference. FLINT introduces three mechanisms: (1) a hardware burst-buffer controller that dynamically coalesces and pipelines HBF reads aiming to utilize existing NAND flash buffers while sustaining high HBF bandwidth, (2) a phantom-plane refresh mechanism, which removes refresh from the critical inference path by moving refresh-related NAND flash operations outside the read foreground back via low-cost resource duplication, and (3) a read-only FTL, which replaces SSD-class support for arbitrary writes with a compact table that translates logical weight bursts to physical HBF locations.

==> Makefile <==
# ============================================================
#  Makefile for HBF CAL paper
#  Usage:
#    make        — full build (pdflatex + bibtex + pdflatex x2)
#    make view   — open PDF (Linux: evince, macOS: open)
#    make clean  — remove auxiliary files
#    make distclean — remove all generated files including PDF
# ============================================================

MAIN    = main
LATEX   = pdflatex
BIBTEX  = bibtex
FLAGS   = -interaction=nonstopmode -halt-on-error

.PHONY: all view clean distclean

all: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex refs.bib
	$(LATEX) $(FLAGS) $(MAIN)
	$(BIBTEX) $(MAIN)
	$(LATEX) $(FLAGS) $(MAIN)
	$(LATEX) $(FLAGS) $(MAIN)

view: $(MAIN).pdf
	@if command -v evince >/dev/null 2>&1; then \
		evince $(MAIN).pdf & \
	elif command -v open >/dev/null 2>&1; then \
		open $(MAIN).pdf; \
	else \
		echo "No PDF viewer found. Open $(MAIN).pdf manually."; \
	fi

clean:
	rm -f $(MAIN).aux $(MAIN).bbl $(MAIN).blg $(MAIN).log \
	       $(MAIN).out $(MAIN).toc $(MAIN).fls $(MAIN).fdb_latexmk \
	       $(MAIN).synctex.gz

distclean: clean
	rm -f $(MAIN).pdf


==> hpca-template.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% -- DO NOT MODIFY -- %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\author{
  \ifdefined\hpcacameraready
    \IEEEauthorblockN{\hpcaauthors{}}
      \IEEEauthorblockA{
        \hpcaaffiliation{} \\
        \hpcaemail{}
      }
  \else
    \IEEEauthorblockN{\normalsize{HPCA \hpcayear{} Submission
      \textbf{\#\hpcasubmissionnumber{}}} \\
      \IEEEauthorblockA{
        Confidential Draft \\
        Do NOT Distribute!!
      }
    }
  \fi 
}

% Heading and footer for title page
\fancypagestyle{camerareadyfirstpage}{%
  \fancyhead{}
  \renewcommand{\headrulewidth}{0pt}
  \fancyhead[C]{
    \ifdefined\aeopen
    \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}    
    \else
      \ifdefined\aereviewed
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \ifdefined\aereproduced
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \parbox[][0mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
    \fi 
    \fi 
    \fi 
    \ifdefined\aeopen 
      \includegraphics[width=12mm,height=12mm]{ae-badges/open-research-objects.pdf}
    \fi 
    \ifdefined\aereviewed
      \includegraphics[width=12mm,height=12mm]{ae-badges/research-objects-reviewed.pdf}
    \fi 
    \ifdefined\aereproduced
      \includegraphics[width=12mm,height=12mm]{ae-badges/results-reproduced.pdf}
    \fi
  }
  %\fancyfoot[L]{\hpcapubid{} \copyright \hpcayear{} IEEE}
  \fancyfoot[C]{}
}
% Heading and footer for remaining pages
\fancyhead{}
\renewcommand{\headrulewidth}{0pt}
%\fancyhead[C]{\hpcayear{} IEEE International Symposium on
% High-Performance Computer Architecture (HPCA)}

\sloppy
\begin{document}
\maketitle

%Enables the camera ready header and footer
\ifdefined\hpcacameraready 
  \thispagestyle{camerareadyfirstpage}
  \pagestyle{empty}
\else
  \thispagestyle{plain}
  \pagestyle{plain}
\fi

\newcommand{\hpcaheight}{0mm}
\ifdefined\eaopen
\renewcommand{\hpcaheight}{12mm}
\fi
  


==> sections/01_introduction.tex <==
\section{Introduction}
\label{sec:intro}

% ---- Paragraph 1: LLM growth and the widening memory wall ----
The trajectory of large language models (LLMs) has been defined by relentless parameter scaling.
From early transformer architectures with hundreds of millions of parameters~\cite{vaswani2017attention, devlin2018bert}, model sizes rapidly expanded to GPT-3 at 175~billion parameters~\cite{brown2020language},
PaLM at  40~billion~\cite{chowdhery2023palm}, and recent open-source models such as Llama~3.1 at 405~billion parameters~\cite{dubey2024llama3}, with closed-source frontier models estimated to be substantially larger~\cite{achiam2023gpt4, comanici2025gemini}.
This scaling has consistently yielded improvements in reasoning, instruction-following, and multi-modal capability, and there is no evidence \gf{that} the trend is abating~\cite{hoffmann2022chinchilla, meta2025llama4}.
The hardware landscape, however, has not kept pace.
As illustrated in Fig.~\ref{fig:memory_wall}, across the NVIDIA
A100, H100, H200, and B200 GPU generations spanning 2020--2025,
peak BF16 tensor-core throughput grew by approximately~$14\times$,
while on-package HBM capacity increased only~$2.4\times$
(80\,GB $\to$ 192\,GB per
GPU)~\cite{nvidia2022a100, nvidia2023h100, nvidia2025b200}.
HBM bandwidth improved at an intermediate pace, from 2.0\,TB/s
to~8.0\,TB/s --- a $4\times$ gain that still trails the compute
scaling ratio by more than~$3\times$.
Off-package interconnects lag even further: PCIe~5.0 delivers
at most 128\,GB/s of bidirectional
bandwidth~\cite{pcisig2019pcie5}, more than~60$\times$ below
HBM bandwidth and several orders of magnitude below aggregate
compute throughput.
The consequence is a widening \emph{memory capacity wall}~\cite{gholami2024airadar}:
for frontier-scale LLMs, the amount of memory available per
accelerator --- not raw compute --- is the dominant bottleneck
for inference deployment.

% ---- Paragraph 2: Existing solutions and HBF ----
At the data-center scale, the community has addressed this
capacity shortfall through model parallelism, distributing
model weights and activations across multiple GPUs via tensor
parallelism~\cite{shoeybi2019megatron, narayanan2021megatron} and
pipeline parallelism~\cite{huang2019gpipe, narayanan2019pipedream}.
These strategies aggregate the HBM capacity of many accelerators
into a larger logical pool and are effective for large-scale
cloud inference.
Yet\gf{,} they are fundamentally ill-suited to \emph{edge inference},
where cost, power envelope, and physical footprint preclude
multi-GPU configurations.
Edge deployment of frontier models thus requires a different
approach to expanding per-node memory capacity.
High-bandwidth flash~(HBF) has recently emerged as a compelling
candidate~\cite{ha2026h3, sandisk2025hbf}.
Inspired by the physical stack of HBM, HBF places NAND flash dies
above a base logic die and connects them via through-silicon
vias~(TSVs), targeting bandwidth comparable to HBM while
offering up to~$16\times$ greater capacity per
package~\cite{ha2026h3}.
SK~Hynix recently proposed the H$^3$ hybrid
architecture~\cite{ha2026h3}, in which HBF is daisy-chained to
HBM on the GPU interposer; an address decoder in the HBM base die
routes accesses to either HBM or HBF within a unified address space,
enabling the GPU to use HBF transparently.
By confining read-only data to HBF, i.e., model weights and shared
pre-computed KV caches~\cite{chan2025cag},
H$^3$ demonstrates up to~$2.69\times$ higher throughput per
\gf{W}att relative to HBM-only configurations~\cite{ha2026h3},
establishing the viability of HBF as a cost-effective GPU memory
extension for large-model edge inference.

% ---- Figure 1: Memory wall ----
\begin{figure}[t]
  \centering
  \begin{tikzpicture}
    \begin{axis}[
      width  = \columnwidth,
      height = 4.6cm,
      xlabel = {GPU Generation},
      ylabel = {Normalized to A100 (\(\times\))},
      xtick  = {1, 2, 3, 4},
      xticklabels = {A100\\{\tiny(2020)},
                     H100\\{\tiny(2022)},
                     H200\\{\tiny(2024)},
                     B200\\{\tiny(2025)}},
      ymode  = log,
      log basis y = 10,
      ymin   = 0.7, ymax = 25,
      ytick  = {1, 2, 4, 8, 14},
      yticklabels = {1$\times$, 2$\times$, 4$\times$, 8$\times$, 14$\times$},
      ymajorgrids = true,
      grid style  = {dashed, gray!40},
      legend style = {at={(0.03,0.97)}, anchor=north west,
                      font=\footnotesize, draw=black!60,
                      fill=white, fill opacity=0.9},
      tick label style = {font=\footnotesize},
      label style       = {font=\small},
      x tick label style = {align=center},
      enlarge x limits   = 0.15,
    ]
    %% HBM Capacity: 80, 80, 141, 192 GB  (norm to 80)
    \addplot[
      color  = blue!70!black,
      mark   = square*,
      mark size = 2.5pt,
      thick,
    ] coordinates {(1,1.00) (2,1.00) (3,1.76) (4,2.40)};
    \addlegendentry{HBM Capacity}

    %% HBM Bandwidth: 2.0, 3.35, 4.8, 8.0 TB/s (norm to 2.0)
    \addplot[
      color  = teal,
      mark   = triangle*,
      mark size = 2.5pt,
      thick,
      dashed,
    ] coordinates {(1,1.00) (2,1.68) (3,2.40) (4,4.00)};
    \addlegendentry{HBM Bandwidth}

    %% Peak BF16 Compute: 312, 989, 989, ~4500 TFLOPS (norm to 312)
    \addplot[
      color  = red!80!black,
      mark   = *,
      mark size = 2.5pt,
      thick,
      dotted,
    ] coordinates {(1,1.00) (2,3.17) (3,3.17) (4,14.42)};
    \addlegendentry{Peak Compute (BF16)}

    \end{axis}
  \end{tikzpicture}
  \caption{
    Normalized GPU compute throughput (BF16 tensor-core),
    HBM capacity, and HBM bandwidth across four NVIDIA GPU
    generations~\cite{nvidia2022a100,nvidia2023h100,nvidia2025b200}.
    All values are normalized to the A100 (80\,GB, 2.0\,TB/s,
    312\,TFLOPS).
    Compute has grown ${\sim}14\times$ while capacity has
    increased only $2.4\times$, creating a widening
    \emph{memory capacity wall}.
  }
  \label{fig:memory_wall}
\end{figure}

% 
